Gravitational waves from bubble collisions and fluid motion in strongly supercooled phase transitions

We estimate the gravitational wave spectra generated in strongly supercooled phase transitions by bubble collisions and fluid motion. We derive analytically in the thin-wall approximation the efficiency factor that determines the share of the energy released in the transition between the scalar field and the fluid. We perform numerical simulations including the efficiency factor as a function of bubble radius separately for all points on the bubble surfaces to take into account their different collision times. We find that the efficiency factor does not significantly change the gravitational wave spectra and show that the result can be approximated by multiplying the spectrum obtained without the efficiency factor by its value at the radius $R_{\rm eff} \simeq 5/\beta$, where $\beta$ is the approximate inverse duration of the transition. We also provide updated fits for the gravitational wave spectra produced in strongly supercooled transitions from both bubble collisions and fluid motion depending on the behaviour of the sources after the collision.

==> reply.tex <==
We thank the referee for their very helpful comments and questions. Please find below our replies and modification we made in the paper:

1. We added footnote 3 clarifying the issue. We cannot, however, agree that this is simply an assumption, since, as we argue, this has behaviour been observed and verified in multiple approaches.

2. We added a new next to last paragraph in sec IV discussing this issue.

3. We added the details of the numerical parameters in footnote 4. We also changed the sentence before it to clarify that we used the scheme given in [45].

4. We now also clarify our R^-3 scaling agrees with the results of Ref. [45] obtained for much weaker transitions. We haven't found a compelling physical argument to justify this scaling, however, we made sure our simulations converge to the same results while using smaller steps so this is unlikely to be just a numerical artifact.

5. We replaced Fig. 3 with a simulation of a much stronger transition with alpha = 20 and gamma_w = 50.

6. In our analysis the transition is parameterised by alpha and beta. The expansion of the universe can be neglected if beta is large enough. This is an assumption in our analysis which we have now clarified in a footnote above Eq (1).

7. We have added a footnote above Eq. (15) to point out that this result agrees with the bubble lifetime distribution derived in [41].

8. Ref. [41] finds the third moment is relevant for RMS fluid velocity and consequently  GW production in the sound shell model. A similar statement should be true in general, and we propose that the typically used average radius should be replaced with the third moment altogether as the quantity relevant for GW generation.

We hope that with these changes and clarifications the paper can be accepted for publication.

Best regards,
Marek Lewicki and Ville Vaskonen






We thank the referee for their further comments. Please find below our replies:

1. As suggested by the referee, we have moved the footnote to the text and clarified the discussion in particular by adding the ranges of $\alpha$ where this behaviour has been observed in numerical simulations.

2. As suggested by the referee, we have modified the new paragraph to make our argument more clear and less definite.

8. As suggested by the referee, we don't anymore denote <R>^{-1/3} by R_* and there should be no confusion regarding using these formulae in earlier literature.

We hope that with these changes and clarifications the paper can be accepted for publication.

Best regards,
Marek Lewicki and Ville Vaskonen



We thank the referee for the comment. We rewrote the paragraph to make more clear the procedure we followed.  Ref. [45] has indeed simulated collisions although in a simplified manner placing two planar shells very close and simulating their further evolution (see their appendix C). We verified in the same manner that the initial conditions in our computation for the evolution of the fluid shell after collision are reasonable.

Best regards,
Marek Lewicki and Ville Vaskonen
